The LDBC Graphalytics Benchmark

In this document, we describe LDBC Graphalytics, an industrial-grade benchmark for graph analysis platforms. The main goal of Graphalytics is to enable the fair and objective comparison of graph analysis platforms. Due to the diversity of bottlenecks and performance issues such platforms need to address, Graphalytics consists of a set of selected deterministic algorithms for full-graph analysis, standard graph datasets, synthetic dataset generators, and reference output for validation purposes. Its test harness produces deep metrics that quantify multiple kinds of systems scalability, weak and strong, and robustness, such as failures and performance variability. The benchmark also balances comprehensiveness with runtime necessary to obtain the deep metrics. The benchmark comes with open-source software for generating performance data, for validating algorithm results, for monitoring and sharing performance data, and for obtaining the final benchmark result as a standard performance report.

==> article.tex <==
\input{graphalytics_spec}

==> tables/related_benchmarks-studies__vldb-summary_large.tex <==
\begin{tabular}[!tb]{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|c|}{Reference} & \multicolumn{2}{c|}{Target System} & \multicolumn{5}{c|}{Design} & \multicolumn{2}{c|}{Includes tests for...} & Other Distinguishing \\ 
\hline
Type & Name [Publication] & \multicolumn{1}{c|}{Structure} & \multicolumn{1}{c|}{Programming} & \multicolumn{1}{c|}{Input} & \multicolumn{1}{c|}{Data.} & \multicolumn{1}{c|}{Algo.} & \multicolumn{1}{c|}{Scalable?} & \multicolumn{1}{c|}{Renewal} & \multicolumn{1}{c|}{Scalability} & \multicolumn{1}{c|}{Robustness} & Features \\ 
\hline
B & \pbox{5cm}{CloudSuite~\cite{DBLP:conf/asplos/FerdmanAKVAJKPAF12 }, \\latest graph elements} & \multicolumn{1}{c|}{D/MC} & \multicolumn{1}{c|}{1 class (PowerGraph)} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Rnd(3)} & \multicolumn{1}{c|}{Exp(1)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Micro-architecture \\ 
\hline
S & Montresor et al.~\cite{DBLP:conf/bigdataconf/ElserM13} & \multicolumn{1}{c|}{D/MC} & \multicolumn{1}{c|}{3 classes} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{Rnd(7)} & \multicolumn{1}{c|}{Exp(1)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Distribution model \\ 
\hline
B & HPC-SGAB~\cite{DBLP:conf/hipc/BaderM05} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(RMAT)} & \multicolumn{1}{c|}{Exp(1+)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & HPC architecture \\ 
\hline
B & Graph500\footnote{http://www.graph500.org} & \multicolumn{1}{c|}{P/MC/GPU} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(RMAT)} & \multicolumn{1}{c|}{Exp(1)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & HPC architecture, industry support \\ 
\hline
B & GreenGraph500\footnote{http://green.graph500.org/greengraph500rules.pdf} & \multicolumn{1}{c|}{P/MC/GPU} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(RMAT)} & \multicolumn{1}{c|}{Exp(1)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Graph500 plus energy \\ 
\hline
B & WGB~\cite{DBLP:conf/wbdb/AmmarO13} & \multicolumn{1}{c|}{D} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{SE+} & \multicolumn{1}{c|}{Exp(RTG)} & \multicolumn{1}{c|}{Exp(several)} & \multicolumn{1}{c|}{1B Edges} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Query type \\ 
\hline
S & {\bf Own work, prior to Graphalytics}~\cite{DBLP:conf/ipps/GuoBVIMW14,DBLP:conf/ccgrid/GuoVIE15,DBLP:conf/sigmod/CapotaHIPEB14} & \multicolumn{1}{c|}{D/MC/GPU} & \multicolumn{1}{c|}{10 classes} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(6,RMAT)} & \multicolumn{1}{c|}{1-stage(5 classes)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{W/S/V/H} & \multicolumn{1}{c|}{No} & Distributed and other platforms, Scalability \\ 
\hline
S & \"Ozsu et al.~\cite{DBLP:journals/pvldb/HanDAOWJ14} & \multicolumn{1}{c|}{D} & \multicolumn{1}{c|}{1 class(Pregel)} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{Exp(5)+Rnd(1)} & \multicolumn{1}{c|}{Exp(4)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{W/S/V/H} & \multicolumn{1}{c|}{No} & Pregel-like features \\ 
\hline
B & \pbox{5cm}{BigDataBench~\cite{DBLP:conf/wbdb/MingLGHYWZ13,DBLP:conf/hpca/WangZLZYHGJSZZLZLQ14}, \\only graph elements} & \multicolumn{1}{c|}{D/MC} & \multicolumn{1}{c|}{1 class (Hadoop)} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Rnd(7)} & \multicolumn{1}{c|}{Rnd(2)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Strong} & \multicolumn{1}{c|}{No} & --- \\ 
\hline
S & Satish et al.~\cite{DBLP:conf/sigmod/SatishSPSPHSYD14} & \multicolumn{1}{c|}{D/MC} & \multicolumn{1}{c|}{6 classes} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(6)+Rnd(1)} & \multicolumn{1}{c|}{Exp(4)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Weak} & \multicolumn{1}{c|}{No} & Optimized code, classes of distributed platforms \\ 
\hline
S & Lu et al.~\cite{DBLP:journals/pvldb/LuCYW14} & \multicolumn{1}{c|}{D} & \multicolumn{1}{c|}{4 classes} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(5c/7)+Rnd(1)} & \multicolumn{1}{c|}{Exp(5c/7)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{Strong} & \multicolumn{1}{c|}{No} & Effects of individual techniques \\ 
\hline
B & GraphBIG~\cite{DBLP:conf/sc/NaiXTKL15} & \multicolumn{1}{c|}{P/MC/GPU} & \multicolumn{1}{c|}{1 class (System G)} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{Exp(5)} & \multicolumn{1}{c|}{Exp(10)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Memory sub-system, System G-like features \\ 
\hline
S & Cherkasova et al.~\cite{conf/icpe/EisenmanCMCFK16} & \multicolumn{1}{c|}{MC} & \multicolumn{1}{c|}{1 class(Galois)} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{Rnd(2)} & \multicolumn{1}{c|}{Exp(5)} & \multicolumn{1}{c|}{---} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{No} & Memory sub-system, Galois-like features \\ 
\hline
B & {\bf LDBC Graphalytics (this work)} & \multicolumn{1}{c|}{D/MC/GPU} & \multicolumn{1}{c|}{10+ classes} & \multicolumn{1}{c|}{SE+} & \multicolumn{1}{c|}{2-stage(10,RMAT,LDBC)} & \multicolumn{1}{c|}{2-stage(6 classes)} & \multicolumn{1}{c|}{1B Edges} & \multicolumn{1}{c|}{Yes} & \multicolumn{1}{c|}{W/S/V/H} & \multicolumn{1}{c|}{Yes} & Distributed and other platforms, industry support \\ 
\hline
\multicolumn{12}{|c|}{Legend: S - Study, B - Benchmark; D - distributed system, P - parallel system, MC - single-node multi-core system, GPU - using GPUs.} \\ 
\hline
\multicolumn{12}{|c|}{Input: {\bf 0} - no parameters; {\bf S} - parameters to define scale; {\bf E} - parameters to define edge properties; {\bf +} - parameters to define other graph properties, e.g., clustering coefficient.} \\ 
\hline
\multicolumn{12}{|c|}{Data[sets]/Algo[rithms]: {\bf Rnd} - reason for selection not explained; {\bf Exp} - selection seems guided by personal expertise; {\bf 1-stage} - data-driven selection; {\bf 2-stage} - 2-stage data-driven and expertise-driven process.} \\ 
\hline
\multicolumn{12}{|c|}{Can test scalability? Weak/Strong/Vertical/Horizontal.} \\ 
\hline
\multicolumn{12}{|c|}{\"---\" - feature not available or unclear from publication(s).} \\ 
\hline
\end{tabular}

==> tex/auditing.tex <==
\chapter{Auditing Rules}
\label{chap:auditing}

The auditing rules are currently under discussion in the LDBC consortium. We welcome feedback from all stakeholders, including both industry and academia organizations.

